Transfer-Meta Framework for Cross-domain Recommendation to Cold-Start Users

Cold-start problems are enormous challenges in practical recommender systems. One promising solution for this problem is cross-domain recommendation (CDR) which leverages rich information from an auxiliary (source) domain to improve the performance of recommender system in the target domain. In these CDR approaches, the family of Embedding and Mapping methods for CDR (EMCDR) is very effective, which explicitly learn a mapping function from source embeddings to target embeddings with overlapping users. However, these approaches suffer from one serious problem: the mapping function is only learned on limited overlapping users, and the function would be biased to the limited overlapping users, which leads to unsatisfying generalization ability and degrades the performance on cold-start users in the target domain. With the advantage of meta learning which has good generalization ability to novel tasks, we propose a transfer-meta framework for CDR (TMCDR) which has a transfer stage and a meta stage. In the transfer (pre-training) stage, a source model and a target model are trained on source and target domains, respectively. In the meta stage, a task-oriented meta network is learned to implicitly transform the user embedding in the source domain to the target feature space. In addition, the TMCDR is a general framework that can be applied upon various base models, e.g., MF, BPR, CML. By utilizing data from Amazon and Douban, we conduct extensive experiments on 6 cross-domain tasks to demonstrate the superior performance and compatibility of TMCDR.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography


Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations
	       

==> Relatedwork.tex <==
\vspace{-0.2cm}\section{Related Work}
% In this section, we will introduce the related work from three aspects: Cross-domain Recommendation, Cold-start, Meta Learning.

% \textbf{Cross-domain Recommendation (CDR)}: With the help of the auxiliary (source) domain, CDR methods can achieve better performance  than single-domain ones. Most existing CDR methods~\cite{singh2008relational,pan2010transfer,he2018general,gao2019cross} aim to improve the overall recommendation performance in the target-domain. Some other approaches have been proposed to make recommendation to cold-start users in the target domain~\cite{mirbakhsh2015improving,man2017cross}. Our study falls into the second category. The most popular method of cold-start in CDR is the Embedding and Mapping method (EMCDR)~\cite{man2017cross}. With the advantage of EMCDR, many
% EMCDR-based approaches~\cite{zhu2018deep,fu2019deeply,kang2019semi} have been proposed. All the EMCDR-based approaches meet the problem of limited overlapping users, while the proposed TMCDR can alleviate the problem for all of them.

% \textbf{Cold-start}: Making recommendation for new users or items is an challenging problem in recommender systems, also named cold-start. Some methods solve cold-start by designing a decision making strategy, such as using contextual-bandits~\cite{li2010contextual,pan2019policy}. Besides, many approaches~\cite{roy2016latent,zhou2011functional} utilize side information to help cold-start stage. In addition, CDR is also a promising solution for cold-start~\cite{man2017cross}, and our study also falls into CDR.

% \textbf{Meta Learning}: It is also named learning to learn, which aims to improve the performance on novel tasks by training on lots of similar tasks. There are various meta learning approaches, e.g., metric-based methods~\cite{vinyals2016matching,snell2017prototypical}, gradient-based methods~\cite{finn2017model,andrychowicz2016learning}. Meta learning leads to an interest in many area, e.g., recommendations~\cite{pan2019warm}, natural language processing~\cite{kiela2018dynamic}, and computer vision~\cite{snell2017prototypical}. The most related work are meta learning for cold-start in recommendations~\cite{vartak2017meta,pan2019warm,du2019sequential,lee2019melu}. In ~\cite{vartak2017meta,pan2019warm,lee2019melu}, they solve cold-start in single domain by using a neural network to directly output parameters of recommender systems or learning model personalized parameters. $s^2$Meta~\cite{du2019sequential} learns a meta-learner to initialize recommender of novel scenarios with few interaction. All of them fall into single domain methods, while the proposed TMCDR is a CDR approach.

In this section, we will introduce the related work from three aspects: Cross-domain Recommendation, Cold-start, Meta Learning.

\textbf{Cross-domain Recommendation (CDR)}: With the help of the auxiliary (source) domain, CDR methods can achieve better performance than single-domain ones. The CDR methods can be divided into two groups: 1) Many existing CDR methods~\cite{singh2008relational,pan2010transfer,he2018general,gao2019cross} aim to improve the overall recommendation performance in the target-domain. 2) Some other approaches have been proposed to make recommendations to cold-start users in the target domain~\cite{mirbakhsh2015improving,man2017cross,zhu2018deep,fu2019deeply,kang2019semi}.  Our study also falls into the second category.

% Many existing CDR methods~\cite{singh2008relational,pan2010transfer,he2018general,gao2019cross} aim to improve the overall recommendation performance in the target-domain. Coordinate System Transfer (CST)~\cite{pan2010transfer} aims to discover the principle coordinates of both users and items in the source data matrices, and transfer them to the target domain in order to reduce the effect of data sparsity. CoNet~\cite{hu2018conet} transfers and combines the knowledge by using cross-connections between feed-forward neural networks, which are used for a base network for each domain. MINDTL~\cite{he2018robust} combines the CF information of the target-domain with the rating patterns extracted from a cluster-level rating matrix in the source-domain.

% Some other approaches have been proposed to make recommendations to cold-start users in the target domain~\cite{mirbakhsh2015improving,man2017cross}. Our study also falls into this category. The most popular method of cold-start in CDR is the Embedding and Mapping method (EMCDR)~\cite{man2017cross}. With the advantage of EMCDR, many
% EMCDR-based approaches~\cite{zhu2018deep,fu2019deeply,kang2019semi} have been proposed. DCDCSR~\cite{zhu2018deep} takes into account the rating sparsity degrees of individual users and items in different domains or systems and uses them to guide the DNN training process for utilizing the rating data more effectively. RC-DFM~\cite{fu2019deeply} extends EMCDR to utilize review texts and item contents. SSCDR~\cite{kang2019semi} is a semi-supervised method which effectively learns the cross-domain relationship even in the case that only a few numbers of labeled data is available. All the EMCDR-based approaches meet the problem of limited overlapping users, while the proposed TMCDR can alleviate the problem for all of them.

\textbf{Meta Learning}: It is also named learning to learn, which aims to improve the performance on novel tasks by training on lots of similar tasks. There are various meta learning approaches, e.g., metric-based methods~\cite{vinyals2016matching,snell2017prototypical}, gradient-based methods~\cite{finn2017model,andrychowicz2016learning}. Our method falls into the second group. The most related work are meta learning for cold-start in recommendations~\cite{vartak2017meta,pan2019warm,du2019sequential,lee2019melu}. However, most of them~\cite{vartak2017meta,pan2019warm,lee2019melu,lu2020meta,dong2020mamo} fall into single-domain recommendation, while we focus on cross-domain recommendation. $s^2$Meta~\cite{du2019sequential} learn common knowledge from multiple available scenarios to help cold-start scenario, which can not solve the cross-domain cold-start problem (two domains).

%The work in~\cite{vartak2017meta} takes a concept of the metric-based meta-learning algorithm in the recommender system to predict whether a user consumes an item or not. $s^2$Meta~\cite{du2019sequential} learns a meta-learner to initialize recommender of novel scenarios with a few interactions. SML~\cite{zhang2020retrain} utilizes meta learning for the retraining task. Some methods~\cite{pan2019warm,lee2019melu,lu2020meta,dong2020mamo,luo2020metaselector} apply MAML~\cite{finn2017model} into recommender systems. MetaEmb~\cite{pan2019warm} utilizes a generator to generate a good initial embedding from side information for all cold items, and the initial embedding is helpful for the warm-up phase. MeLU~\cite{lee2019melu} applies MAML~\cite{finn2017model} to address cold-star problem (warm-up phase), which learns personalized model parameters from historical interaction for each user. MetaHIN~\cite{lu2020meta} and MAMO~\cite{dong2020mamo} share the similar idea with MeLU. In MetaSelector~\cite{luo2020metaselector}, a model selector is trained via meta-learning to select the best single model for each user with the user-specific historical data. However, most of them~\cite{vartak2017meta,pan2019warm,lee2019melu,lu2020meta,dong2020mamo} fall into single-domain recommendation, while we focus on cross-domain recommendation. $s^2$Meta~\cite{du2019sequential} learn common knowledge from multiple available scenarios to help cold-start scenario, which can not solve the cross-domain cold-start problem (two domains).

\textbf{Cold-start}: Making recommendations for new users or items is a challenging problem in recommender systems, also named cold-start. There are two kinds of methods to solve the cold-start problem. Auxiliary information is helpful to the cold-start stage. There are various ways to use auxiliary information, e.g., user attributes~\cite{seroussi2011personalised,li2019zero}, item attributes~\cite{mo2015image,saveski2014item}, knowledge graph~\cite{wang2018ripplenet}, samples in an auxiliary domain~\cite{man2017cross}. In addition, utilizing samples in an auxiliary domain is also known as cross-domain recommendation (CDR) which is a promising solution for cold-start~\cite{man2017cross}, and our study also falls into CDR. %Usually, with samples in an auxiliary domain, the CDR methods designed for the cold-start problem can achieve much better results than other kinds of cold-start methods. Thus, in this paper, following most CDR work~\cite{man2017cross,kang2019semi}, we only compare our method with CDR approaches.

